Multiwavelength analysis and the C IV {\lambda}1549 {\AA} emission line behavior from 2008 to 2020 of the FSRQ B2 1633+382

The flat-spectrum radio quasar B2 1633+382 (4C 38.41) has been monitored for several years and has presented correlated variability in multiple wavelengths. In this article, we are performing different analyses for multiple frequencies, from gamma-rays to radio, as well as, the C IV ${\lambda}$1549 {\AA} emission line and the ${\lambda}$1350 {\AA} continuum. Using the non-thermal dominance parameter, we separated the C IV and the continuum light curves for when the dominant source of continuum is the accretion disk or the jet. We found a correlation at a delay consistent with zero between the line and the continuum dominated by disk emission indicating a very small broad-line region (BLR). From the resulting delay between the 15 GHz and gamma-rays, we estimated the distance of the gamma-ray emission region from the jet apex to be $\sim$37 pc. The C IV flux decreases when the continuum and gamma-rays increase at some of the high activity periods. The C IV profile presents a larger variable component in its blue wing. The relation between the luminosities of C IV and the continuum does not completely follow the relation for a quasar sample. Our results lead us to propose an outflow of BLR material in the jet-flow direction, a gamma-ray production through magnetic reconnection for the flaring event of mid-2011, and that there is not enough BLR material close to the radio core to be easily ionized by the non-thermal continuum.

==> Artículo (ArXiv)/Table1_flux.tex <==
\begin{table}[htbp]
\centering
\caption{\tablenotemark{*}Sample of the flux measurements for the $\lambda$1350 \AA\ continuum and the C IV $\lambda$1549 \AA\ emission line.}
\begin{tabular}{ccccc}
\hline
\hline
\multirow{2}{*}{JD-2450000} & {Flux Continuum $\lambda$1350 \AA\ } &  {Flux C IV $\lambda$1549 \AA\ } \\
 & $\times10^{-15}\, erg\, s^{-1}cm^{-2}\, {\rm \AA}^{-1}$ & $\times10^{-15}\, erg\, s^{-1}cm^{-2}$ \\
\hline
4745.63 &    12.69 $\pm$    1.62 &    293.74 $\pm$    21.51 \\
4746.63 &    13.31 $\pm$    2.02 &    304.57 $\pm$    26.74 \\
4747.63 &    13.94 $\pm$    2.51 &    255.50 $\pm$    32.97 \\
4748.64 &    15.40 $\pm$    2.71 &    287.53 $\pm$    35.53 \\
4767.60 &    13.64 $\pm$    1.72 &    224.82 $\pm$    22.29 \\
4768.59 &    11.08 $\pm$    0.78 &    233.48 $\pm$    10.09 \\
4769.58 &    12.44 $\pm$    1.38 &    265.99 $\pm$    18.08 \\
4770.58 &    12.26 $\pm$    1.68 &    241.12 $\pm$    22.10 \\
4771.58 &    13.43 $\pm$    1.84 &    269.56 $\pm$    24.21 \\
4772.58 &     9.56 $\pm$    0.82 &    210.70 $\pm$    10.72 \\
\hline
\end{tabular}
\tablenotetext{*}{The complete table is available in a machine-readable form in the online journal.}
\label{Table_flux}
\end{table}



==> Artículo (ArXiv)/Table2_cc.tex <==
\begin{table}
\centering
\caption{Cross-correlation results for the full light curves given in time delays (days) with their uncertainty at 90\% confidence level. All delays have correlations at the $\geq$ 99\% significance level. The results are only shown for the cross-correlation analyses in which the delays are not aliases. All cross-correlations are performed in the order stated in this table e.g. if the delay is positive then the first band leads the second and if the delay is negative the first band lags the second.}

\begin{tabular}{lc}
\hline
\hline
                Bands &         Delay                                 \\
\hline
        1 mm versus X-rays &           -120.4 $\pm$  16.9             \\
        15 GHz versus 1 mm &           -38.9 $\pm$              16.3  \\
     15 GHz versus 1350\AA &  No correlation                          \\
        15 GHz versus C IV &            83.4 $^{+23.9}_{-21.4}$       \\
  15 GHz versus Gamma-rays &           -69.5 $\pm$               8.7  \\
      15 GHz versus X-rays &  No correlation                          \\
1350\AA\ versus Gamma-rays &            -7.4 $\pm$               8.7  \\
      1350\AA\ versus C IV &  No correlation                          \\
    1350\AA\ versus X-rays &  No correlation                          \\
      1350\AA\ versus 1 mm &  No correlation                          \\
    C IV versus Gamma-rays &  No correlation                          \\
        C IV versus X-rays &  No correlation                          \\
          C IV versus 1 mm &  No correlation                          \\
             V versus 1 mm &            26.6 $\pm$              16.3  \\
           V versus 15 GHz &            82.4 $\pm$               4.7  \\
         V versus 1350\AA\ &             0.0 $\pm$               5.9  \\
             V versus C IV &  No correlation                          \\
       V versus Gamma-rays &             0.7 $\pm$               8.7  \\
           V versus X-rays &  No correlation                          \\
    Gamma-rays versus 1 mm &            19.3 $\pm$              16.3  \\
  Gamma-rays versus X-rays &  No correlation                          \\
\hline
\end{tabular}

\label{Table_CC}

\end{table}


==> Artículo (ArXiv)/Table3_Fvar.tex <==
\begin{table}
\centering
\caption{Fractional variability (F$_{\text{var}}$) of the multiple wave bands.}

\begin{tabular}{lc}
\hline
\hline
                Bands &         F$_{\text{var}}$  \\
\hline
         15~GHz &      0.220 $\pm$ 0.001  \\
         1~mm &        0.449 $\pm$ 0.005  \\
         V-band &      0.580 $\pm$ 0.001  \\
        1350\AA\ &     0.486 $\pm$ 0.005 \\
          X-rays &     0.533 $\pm$ 0.008 \\
      Gamma-rays &     1.142 $\pm$ 0.013 \\
\hline
\end{tabular}

\label{Table_Fvar}

\end{table}


==> Artículo (ArXiv)/Table4_corr-periods.tex <==
\begin{table}
\centering
\caption{Linear fitting and Spearman correlation rank test (SCRT) results for the luminosity relations of the full period of observations and of the separated periods defined in Section \ref{sec:var}. The column Continuum refers to the dominant source of UV-continuum in the corresponding period, the flag D refers to disk dominated while J refers to jet dominated. If there is no flag, it means that there is not clear dominant source in the corresponding period. For more details see Section \ref{sec:LumRel}.}
\begin{tabular}{lccccc}
\hline
\hline
                         &       \multicolumn2c{Linear Fit} &        \multicolumn2c{SCRT} & \\
                 Periods &           Slope &        P-value &     $\rho$ &       P-value  & Continuum\\
\hline

  	            Full &     $0.06\pm0.01$ &          1.000 &      -0.10 &         0.045  &  \\


                    Full &     $0.40\pm0.02$ &          1.000 &       0.29 &         0.000  & D\\
                      P1 &     $0.55\pm0.07$ &          0.997 &       0.20 &         0.084  & D\\
		      P3 &     $0.31\pm0.03$ &          1.000 &       0.12 &         0.511  & D\\
		      P5 &     $0.48\pm0.07$ &          0.999 &       0.37 &         0.014  & D\\

                    Full &     $0.14\pm0.03$ &          1.000 &       0.13 &         0.122  & J\\
		      P2 &    $-0.10\pm0.03$ &          0.995 &      -0.47 &         0.002  & J\\
		      P4 &     $0.05\pm0.05$ &          0.221 &       0.13 &         0.350  & J\\
                      P7 &    $-0.05\pm0.09$ &          0.866 &      -0.22 &         0.253  & J\\

		      P6 &    $-0.10\pm0.03$ &          1.000 &      -0.22 &         0.037  &  \\
		      
\hline
\end{tabular}
\label{Table_corr-periods}
\end{table}

